HYPERTILING -- a high performance Python library for the generation and visualization of hyperbolic lattices

HYPERTILING is a high-performance Python library for the generation and visualization of regular hyperbolic lattices embedded in the Poincar\'e disk model. Using highly optimized, efficient algorithms, hyperbolic tilings with millions of vertices can be created in a matter of minutes on a single workstation computer. Facilities including computation of adjacent vertices, dynamic lattice manipulation, refinements, as well as powerful plotting and animation capabilities are provided to support advanced uses of hyperbolic graphs. In this manuscript, we present a comprehensive exploration of the package, encompassing its mathematical foundations, usage examples, applications, and a detailed description of its implementation.

==> tex/code-example.tex <==
% this is from Manuels PhD thesis, to be used as an example
\begin{figure}
	%	\small
	\setstretch{1.15}
	%	\hrule height \phaserulewidth
	\begin{algorithmic}
		\State \textbf{Input}: set $G$ of $N=L^d$ sites in $\left[0,L\right)^d$
		\State \textbf{Parameters}:
		\begin{itemize}
			\item $M_c, M_r\geq 2$ number of connection and rewiring layers
			\item $q=q_1+\ldots+q_{M_c}$ coordination number \Comment{$q_i\geq 2$}
			\item $r_1, \ldots, r_{M_c+M_r} \in \mathbb{R}^d$ cell displacement vectors
			\item $\ell$ linear cell size \Comment{typically $\ell\approx 8$}
			\item $s$ number of rewiring attempts per cell and layer
			\item $T$ initial SA temperature (optional)
		\end{itemize}
		\State \textbf{Complexity}: $\mathcal{O}(sqM_rN)$
		\phase{Initial Connections}
		\For{$a=1$ \textbf{to} $M_c$}\Comment{iterate over connection layers}
		\State subdivide spatial domain into cells $\mathcal{K}_{a,n}$ 
		\State of size $\ell^d$, displaced by $r_a$ w.r.t.~the origin
		\ForAll{cells $\mathcal{K}_{a,n}$}
		\State \textbf{call} \textsc{Connect\_Subgraph}(sites in $\mathcal{K}_{a,n}$; $q_a$)
		\EndFor
		\EndFor
		\phase{Dynamical Rewiring}
		\For{$a=1$ \textbf{to} $M_r$}\Comment{iterate over rewiring layers}
		\State subdivide spatial domain into cells $\mathcal{K}_{a,n}$ 
		\State of size $\ell^d$, displaced by $r_{a+M_c}$ w.r.t.~the origin
		\ForAll{open cells $\tilde{\mathcal{K}}_{a,n}$} 
		\For{$ b=1 $ \textbf{to} $s\cdot q$} \Comment{number of repetitions per cell}
		\State $i$, $j$ $\leftarrow$ two random sites $\in G$
		\State $l$ $\leftarrow$ random neighbour of $i$
		\State $k$ $\leftarrow$ random neighbour of $j$
		\If{\textbf{not} any duplicates in $\{i,j,k,l\}$ \\ \textbf{and} $i$ \textbf{is not} neighbour of $j$ \\
			\textbf{and} $k$ \textbf{is not} neighbour of $l$}
		\State \textbf{call} \textsc{Rewiring\_Attempt}($ {i,j,k,l} $; $ T $)
		\EndIf
		\EndFor
		\EndFor
		\State decrease temperature (if not initially zero)
		\EndFor
		\State \textbf{repeat} Phase 2 \textbf{until} desired locality is reached
	\end{algorithmic}
	\hrule height \phaserulewidth
	\caption[Pseudocode for the construction of the CC lattice]{\textbf{Pseudocode for the construction of the CC lattice.} The subroutines \textsc{Connect\_Subgraph} and \textsc{Rewiring\_Attempt} are described in Figures~\ref{alg:Helper1} and \ref{alg:Helper2}.}
	\label{alg:AlgorithmMain}
\end{figure}


\begin{figure}
	%	\small
	\setstretch{1.15}
	\hrule height \phaserulewidth
	\begin{algorithmic}
		\Statex
		\Procedure{Connect\_Subgraph}{set of sites $G$; $q$}
		\State \textsc{Shuffle} $G$
		\State $l_G$ $ \leftarrow $ length of G
		\For{$i=1$ \textbf{to} $l_G$}
		\For{$j=1$ \textbf{to} $q/2$}
		\State $k\leftarrow\mod(i+j,l_G) $ \Comment{cyclic connections}
		\State Add bond from site $G(i)$ to site $G(k) $
		\EndFor
		\EndFor
		\State \Return
		\EndProcedure
		\Statex
	\end{algorithmic}
	\hrule height \phaserulewidth
	\caption[Pseudocode for CC code subroutines (1)]{\textbf{Pseudocode for the subroutines (1).} This function cyclically connects a set of points. Note that a call to this subroutine might produce a connection already produced by a previous call, in which case a reshuffle is necessary.}
	\label{alg:Helper1}
\end{figure}

\begin{figure}
	%	\small
	\setstretch{1.15}
	\hrule height \phaserulewidth
	\begin{algorithmic}
		\Statex
		\Procedure{Rewiring\_Attempt}{sites $i,j,k,l$; $T$}
		\State $d_A$ $\leftarrow$ distance($i,l$) + distance($j,k$) \Comment{respecting p.b.c}
		\State $d_B$ $\leftarrow$ distance($i,j$) + distance($k,l$)
		\State $\Delta H \leftarrow d_B-d_A$ \Comment{cost function, Equation~\eqref{eq:cost}}
		\State Draw random number $r\in[0,1)$
		\If{$r<\min(1,\mathrm{e}^{-\Delta H / T})$}
		\State Remove bond from $i$ to $l$
		\State Remove bond from $j$ to $k$
		\State Add bond from $i$ to $j$
		\State Add bond from $k$ to $l$
		\EndIf
		\State \Return
		\EndProcedure
		\Statex
	\end{algorithmic}
	\hrule height \phaserulewidth
	\caption[Pseudocode for CC code subroutines (2)]{\textbf{Pseudocode for the subroutines (2).} This function attempts a rewiring step by choosing four sites which are mutually connected and comparing the combined bond lengths in the old and new configuration.}
	\label{alg:Helper2}
\end{figure}


==> tex/existing.tex <==
% !TeX root = ../main.tex



==> tex/scope.tex <==
% !TeX root = main.tex

\subsection{Existing Implementations}


\begin{itemize}
\item 2002, David E. Joyce, Java, \url{http://aleph0.clarku.edu/~djoyce/poincare/PoincareB.html};  \url{https://mathcs.clarku.edu/~djoyce/poincare/Polygon.java}

\item 2003, Miodrag Sremcevic, Radmila Sazdanovic, Srdjan Vukmirovic, Mathematica, \url{https://library.wolfram.com/infocenter/MathSource/4540/}

\item 2004, Don Hatch, Java,  \url{http://www.plunk.org/~hatch/HyperbolicApplet/HyperbolicApplet.jar}

\item 2005, Ajit Datar, , \url{https://sourceforge.net/projects/hyperart/};    \url{https://web.archive.org/web/20170301081114/http://www.d.umn.edu/~data0003/Projects/HyperArt/thesis.pdf} , (based on Dunham's Hyperbolic Symmetry, 1986  \cite{DUNHAM1986139})

\item 2007, Dmitry Brant, , \url{https://dmitrybrant.com/files/Tessellation.zip};  \url{https://dmitrybrant.com/2007/01/24/hyperbolic-tessellations}

\item 2012, Kean Walmsley, AutoCAD using .NET,  \url{https://through-the-interface.typepad.com/through_the_interface/2012/01/generating-hyperbolic-tessellations-inside-autocad-using-net.html}

\item 2017, Stephan Mertens and Cristopher Moore, C++, personal communication (now in \texttt{hyperlibrary/other\_codes/mertens2017})

\item 2018, , F\#,  \url{https://github.com/heidisu/hyperbolic} , (based on Dunham's Hyperbolic Symmetry, 1986 \cite{DUNHAM1986139})

\item 2019, , OpenSCAD, \url{https://www.thingiverse.com/thing:3548303};  \url{https://content.instructables.com/ORIG/FEF/DMYM/K2OXD74W/FEFDMYMK2OXD74W.pdf}

\item 2020, Emrys-Merlin, Ruby + gnuplot, \url{https://github.com/Emrys-Merlin/hyperbolic-tessellation}

\item 2021, looeee Lewy Blue, JavaScript, \url{https://github.com/looeee/hyperbolic-tiling} (based on Dunham's Hyperbolic Symmetry, 1986 \cite{DUNHAM1986139})
\end{itemize}


% merge this into the introduction:
%\subsection{Applications}
%
%
%
%\begin{itemize}
%
%\item Edge states dominance effect on topological phases:
%  Topological Hyperbolic Lattices
%Sunkyu Yu, Xianji Piao, and Namkyoo Park
%Phys. Rev. Lett. 125, 053901 – Published 29 July 2020
%  \url{https://link.aps.org/doi/10.1103/PhysRevLett.125.053901}
%\cite{PhysRevLett.125.053901}
%
%\item Constraint percolation on hyperbolic lattices
%Jorge H. Lopez and J. M. Schwarz
%Phys. Rev. E 96, 052108 – Published 6 November 2017
%\textbf{10 layers, Wierstrass, self-implemented, ref: Dunham}
%  \url{https://link.aps.org/doi/10.1103/PhysRevE.96.052108}
%\cite{PhysRevE.96.052108}
%
%\item Percolation on hyperbolic lattices
%Seung Ki Baek, Petter Minnhagen, and Beom Jun Kim
%Phys. Rev. E 79, 011124 – Published 23 January 2009
%\textbf{layer size formula}
%  \url{https://link.aps.org/doi/10.1103/PhysRevE.79.011124}
%\cite{PhysRevE.79.011124}
%
%\item Percolation thresholds in hyperbolic lattices
%Stephan Mertens and Cristopher Moore
%Phys. Rev. E 96, 042116 – Published 9 October 2017
%\textbf{self-implemented C++ code; sudocode} supposed available in \url{https://wasd.urz.uni-magdeburg.de/mertens/research/percolation/} but not to be found -- emailed to Jefferson when requested
%\cite{PhysRevE.96.042116}
%
%\item Crossing on hyperbolic lattices
%Hang Gu and Robert M. Ziff
%Phys. Rev. E 85, 051141 – Published 29 May 2012
%\textbf{Enhanced or Extended Binary Tree (EBT); layer size formula}
%\url{https://link.aps.org/doi/10.1103/PhysRevE.85.051141}
%\cite{PhysRevE.85.051141}
%
%\item Bootstrap Percolation and Kinetically Constrained Models on Hyperbolic Lattices
%    François Sausset, Cristina Toninelli, Giulio Biroli \& Gilles Tarjus 
%Journal of Statistical Physics volume 138, pages 411–430 (2010)
%\textbf{algorithm based on {margenstern2006algorithmic}}
%\url{https://link.springer.com/article/10.1007/s10955-009-9903-1}
%\cite{sausset2010bootstrap}
%
%\item Lattice setup for quantum field theory in AdS2
%Richard C. Brower, Cameron V. Cogburn, A. Liam Fitzpatrick, Dean Howarth, and Chung-I Tan
%Phys. Rev. D 103, 094507 – Published 14 May 2021
%\textbf{self-implemented C code and Mathematica}; review of hyperbolic geometry
%\url{https://link.aps.org/doi/10.1103/PhysRevD.103.094507}
%\cite{PhysRevD.103.094507}
%
%\item Tricritical point of the J1--J2 Ising model on a hyperbolic lattice
%R. Krcmar, T. Iharagi, A. Gendiar, and T. Nishino
%Phys. Rev. E 78, 061119 – Published 17 December 2008
%\url{https://link.aps.org/doi/10.1103/PhysRevE.78.061119}
%\cite{PhysRevE.78.061119}
%
%\item Phase Transition of the Ising Model on a Hyperbolic Lattice
%Takatsugu Iharagi1, Andrej Gendiar2,3, Hiroshi Ueda4, and Tomotoshi Nishino1
%J. Phys. Soc. Jpn. 79, 104001 (2010)
%\url{https://doi.org/10.1143/JPSJ.79.104001}
%\cite{JPSJ.79.104001}
%
%\item Ising model on a hyperbolic lattice studied by the corner transfer matrix renormalization group method
%R Krcmar1, A Gendiar1, K Ueda2 and T Nishino2 
%J. Phys. A: Math. Theor. 41 125001 (2008)
%\url{https://doi.org/10.1088/1751-8113/41/12/125001}
%\cite{Krcmar_2008}
%
%\end{itemize}

